A Predictive Discrete-Continuum Multiscale Model of Plasticity With Quantified Uncertainty

Multiscale models of materials, consisting of upscaling discrete simulations to continuum models, are unique in their capability to simulate complex materials behavior. The fundamental limitation in multiscale models is the presence of uncertainty in the computational predictions delivered by them. In this work, a sequential multiscale model has been developed, incorporating discrete dislocation dynamics (DDD) simulations and a strain gradient plasticity (SGP) model to predict the size effect in plastic deformations of metallic micro-pillars. The DDD simulations include uniaxial compression of micro-pillars with different sizes and over a wide range of initial dislocation densities and spatial distributions of dislocations. An SGP model is employed at the continuum level that accounts for the size-dependency of flow stress and hardening rate. Sequences of uncertainty analyses have been performed to assess the predictive capability of the multiscale model. The variance-based global sensitivity analysis determines the effect of parameter uncertainty on the SGP model prediction. The multiscale model is then constructed by calibrating the continuum model using the data furnished by the DDD simulations. A Bayesian calibration method is implemented to quantify the uncertainty due to microstructural randomness in discrete dislocation simulations (density and spatial distributions of dislocations) on the macroscopic continuum model prediction (size effect in plastic deformation). The outcomes of this study indicate that the discrete-continuum multiscale model can accurately simulate the plastic deformation of micro-pillars, despite the significant uncertainty in the DDD results. Additionally, depending on the macroscopic features represented by the DDD simulations, the SGP model can reliably predict the size effect in plasticity responses of the micropillars with below 10% of error

==> Makefile <==
all:	all_texs

clean: clean_texs clean_exec

clean_texs:
	rm -f *.aux
	rm -f *.log
	rm -f *.dvi
	rm -f *.toc
	rm -f *.blg
	rm -f *.bbl
	rm -f sgp_dd_bayes*.ps
	rm -f *.out
	rm -f *.nav
	rm -f *.snm
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind	
	rm -f *.fdb_latexmk
	rm -f *.fls	
	rm -f *.synctex.gz

clean_exec:
	rm -f *~

#OBJS_convert = \
#	rawfigs/xyz.eps \
#	rawfigs/abc.eps

# $(OBJS_convert)

all_texs:
	pdflatex 	sgp_dd_bayes.tex
	pdflatex 	sgp_dd_bayes.tex
	bibtex sgp_dd_bayes
	pdflatex 	sgp_dd_bayes.tex
	pdflatex 	sgp_dd_bayes.tex	
	

.SUFFIXES: .eps .png .jpg

%.eps: %.png
	convert $< $(basename $<).eps

%.eps: %.jpg
	convert $< $(basename $<).eps

